A Multimodal Single-Branch Embedding Network for Recommendation in Cold-Start and Missing Modality Scenarios

Most recommender systems adopt collaborative filtering (CF) and provide recommendations based on past collective interactions. Therefore, the performance of CF algorithms degrades when few or no interactions are available, a scenario referred to as cold-start. To address this issue, previous work relies on models leveraging both collaborative data and side information on the users or items. Similar to multimodal learning, these models aim at combining collaborative and content representations in a shared embedding space. In this work we propose a novel technique for multimodal recommendation, relying on a multimodal Single-Branch embedding network for Recommendation (SiBraR). Leveraging weight-sharing, SiBraR encodes interaction data as well as multimodal side information using the same single-branch embedding network on different modalities. This makes SiBraR effective in scenarios of missing modality, including cold start. Our extensive experiments on large-scale recommendation datasets from three different recommendation domains (music, movie, and e-commerce) and providing multimodal content information (audio, text, image, labels, and interactions) show that SiBraR significantly outperforms CF as well as state-of-the-art content-based RSs in cold-start scenarios, and is competitive in warm scenarios. We show that SiBraR's recommendations are accurate in missing modality scenarios, and that the model is able to map different modalities to the same region of the shared embedding space, hence reducing the modality gap.

==> algorithms/itemsbrec.tex <==
\makeatletter
\newdimen\commentwd
\let\oldtcp\tcp
\def\tcp*[#1]#2{% only support one style for simplicity
    \setbox0\hbox{#2}%
    \ifdim\wd\z@>\commentwd\global\commentwd\wd\z@\fi
    \oldtcp*[r]{\leavevmode\hbox to \commentwd{\box0\hfill}}
}


\def\mytcp*[#1]#2{% only support one style for simplicity
    \setbox0\hbox{#2}%
    \ifdim\wd\z@>\commentwd\global\commentwd\wd\z@\oldtcp*[r]{\leavevmode\hbox to \commentwd{\box0\hfill}}\fi
    \ifdim\wd\z@<\commentwd\oldtcp*[r]{\leavevmode\hbox to \wd\z@{\box0\hfill}}\fi
}

\let\oldalgorithm\algorithm
\def\algorithm{\oldalgorithm
\global\commentwd\z@
\expandafter\ifx\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname\relax\else
\global\commentwd\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname
\fi
}
\let\oldendalgorithm\endalgorithm
\def\endalgorithm{\oldendalgorithm
\immediate\write\@auxout{\gdef\expandafter\string\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname{%
\the\commentwd}}}
    
    %\centering
    \begin{algorithm*}
        \DontPrintSemicolon
        \caption{Pseudocode for computing the batch loss function in \sbrecItem models}\label{alg:batchloss}
            \SetKwInOut{Input}{Input}            \SetKwInOut{Output}{Output}
            \SetKwFunction{negSampling}{negSampling}
            \SetKwFunction{randomSampling}{randomSampling}
            \Input{
                %$B = \{b | b \subset \{(u_i, i_j) | P_{ij}=1\}\}$: Batches of user--item training interactions\\
                $b \subset \{(u_i, i_j) | R_{ij}=1\}$: Batch of user--item training interactions\\
                $n_\text{neg}$: Number of negatives per interaction\\
                $\mathcal{M}^\text{item}$: Item training modalities\\
                \texttt{ctrEmbs}: Whether to use contrastive loss or not\\
                $\lambda, \tau$: Weight and temperature of contrastive loss
            }
            \Output{$\mathcal{L}$: Loss for the batch
            \vspace{-.9pt}}
%\scalebox{0.9}{
                $\mathcal{L}_\text{BPR} \leftarrow 0$ \tcp*[l]{Reset BPR Loss}
                $\mathcal{L}_\text{SInfoNCE} \leftarrow 0$ \tcp*[l]{Reset contrastive loss}
                \uIf{\texttt{ctrEmbs}}{$n_\text{mod} \leftarrow 2$}
                \Else{$n_\text{mod} \leftarrow 1$}
                \For{$(u_i, i_j)\in b$}{
                    $\mathbf{e_{i}} \leftarrow h(u_i)$\tcp*[l]{Embed user $u_i$}
                    $\mathcal{N}_{ij}\leftarrow$ \negSampling{$u_i, i_j, R$}\tcp*[l]{Sample negatives}
                    $\mathcal{M}_{ij}\leftarrow$ \randomSampling{$\mathcal{M}^{\text{item}}$}\tcp*[l]{Sample $n_\text{mod}$ training modalities}
                    %\For{$m \in \mathcal{M}_{ij}$}{
                    $\mathbf{e_{j}} \leftarrow \frac{1}{n_\text{mod}}\sum_{m\in \mathcal{M}_{ij}}g(m_j)$\tcp*[l]{Embed positive item $i_j$ with single-branch $g$ on modalities $\mathcal{M}_{ij}$}
                    $\hat{y}_{ij} \leftarrow \mathbf{e_{i}}\cdot\mathbf{e_{j}}$\tcp*[l]{Compute positive logit}
                    \For{$i_k \in \mathcal{N}_{ij}$}{
                        $\mathbf{e_{k}} \leftarrow \frac{1}{n_\text{mod}}\sum_{m\in \mathcal{M}_{ij}}g(m_k)$\tcp*[l]{Embed item $i_k$ with single-branch $g$ on modalities $\mathcal{M}_{ij}$}
                        $\hat{y}_{ik} \leftarrow \mathbf{e_{i}}\cdot\mathbf{e_{k}}$\tcp*[l]{Compute negative logit}
                        $\mathcal{L}_\text{BPR} \leftarrow \mathcal{L}_\text{BPR} + \ln{\sigma(\hat{y}_{ij} - \hat{y}_{ik})}$ \tcp*[l]{Accrete BPR loss}
                    }
                    \If{\texttt{ctrEmbs}}{
                                $\mathcal{L}_\text{SInfoNCE} \leftarrow \mathcal{L}_\text{SInfoNCE} - \ln{\frac{\mathrm{e}^{(g(m^{j}_1) \cdot g(m^{j}_2))/\tau}}{\sum_{k \in \{j\}\cup \mathcal{N}_{ij}}\mathrm{e}^{(g(m^{j}_1) \cdot g(m^{k}_2))/\tau}}} - \ln{\frac{\mathrm{e}^{(g(m^{j}_2) \cdot g(m^{j}_1))/\tau}}{\sum_{k \in \{j\}\cup \mathcal{N}_{ij}}\mathrm{e}^{(g(m^{j}_2) \cdot g(m^{k}_1))/\tau}}}$\mytcp*[l]{Accrete contrastive loss}
                    }
                    $\mathcal{L} \leftarrow \mathcal{L}_\text{BPR} + \lambda \mathcal{L}_\text{SInfoNCE}$
                }
            %}
    \end{algorithm*}

==> figures/fig-cold-start-description.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cold-start-user.pdf}
        \caption{user cold-start}
        \label{fig:exp:cold-start-user}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cold-start-item.pdf}
        \caption{item cold-start}
        \label{fig:exp:cold-start-item}
    \end{subfigure}
    %\hfill
    \vspace{-0.5em}
    \caption{The 
    % three
    two
    different cold-start scenarios. The whole square represents all users and items of a dataset, which are split into train, validation and test sets. This is indicated with the different subregions labeled \textit{train}, \textit{val} and \textit{test}, respectively. In (a), users are split randomly such that no user exists in more than one split. Similarly, in (b), no item exists in more than one split. 
    }
    \label{fig:exp:cold-start}
\end{figure}

==> figures/fig-embedding-space.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/projection_5mod_input.pdf}
        \caption{input}
        \label{fig:projection:input}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/projection_5mod_output.pdf}
        \caption{output}
        \label{fig:projection:output}
    \end{subfigure}
    \caption{t-SNE projected embeddings before and after \sbrec. While the different modalities can be differentiated at the model input (a), due to \sbrec, all modalities end up in the same feature space (b).}
    \label{fig:projection}
\end{figure}

==> figures/fig-regularization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/regularization_sweep.pdf}
    \caption{Different combinations of the regularization temperature and regularization loss weight. For regularization weight $0$, the minor performance differences can be explained by randomness in the model initialization.}
    \label{fig:regularization}
%\vspace{-0.6em}
\end{figure}

==> tables/tab_results.tex <==
\begin{center}
\begin{table*}[!htb]
    \centering
    \begin{tabular}{lll|rrr|rrr|rrr}
        %\toprule
          & & & \multicolumn{3}{c|}{Warm} & \multicolumn{6}{c}{Cold} \\
          & & & & & & \multicolumn{3}{c|}{Item} & \multicolumn{3}{c}{User} \\
          & & & \mlonem & \onion & \amazonvid & \mlonem & \onion & \amazonvid &  \mlonem & \onion & \amazonvid \\
          \multirow{2}{*}{Baselines} & Pop & NDCG & & & & & & & & &\\%\cline{2-6}
          & Rand & NDCG & & & & & & & & &\\\midrule
         \multirow{2}{*}{CF} & \bpr & NDCG & & & & & & & & &\\%\cline{2-6}
          & \dmf & NDCG & & & & & & & & &\\\midrule
         \multirow{6}{*}{CBR} & \multirow{2}{*}{\dropoutnet} &NDCG & & & & & & & & &\\%\cdashline{3-6}
          & &$\Delta$NDCG & & & & & & & & &\\\cdashline{2-12}
          & \multirow{2}{*}{\clcrec} &NDCG & & & & & & & & &\\
          & &$\Delta$NDCG & & & & & & & & &\\\cdashline{2-12}
          & \multirow{2}{*}{\sbrec 2 mod.} &NDCG & & & & & & & & &\\
          & &$\Delta$NDCG & & & & & & & & &\\\cdashline{2-12}
          & \multirow{2}{*}{\sbrec $\geq 3$ mod.} &NDCG & & & & & & & & &\\
          & &$\Delta$NDCG & & & & & & & & &\\
        \bottomrule
    \end{tabular}
    \vspace{0.6em}
    \caption{Evaluation results \wrt NDCG@10. Bold indicates the best performing CF model and the best performing CBR model. For CBR, $\Delta$ indicates the percentage change over the best performing CF model. The sign $\dagger$ indicates significant improvement of the best performing CBR model over the best performing CF model, while $\ddag$ significant improvement over the other CBR models.}
    \label{tab:results-overview}
\end{table*}
\end{center}

==> tables/tab_results_ap.tex <==
\begin{center}
\begin{table*}[!htb]\scalebox{0.9}{
    \centering
    \begin{tabular}{lll|rrr|rrr|rr}
        %\toprule
          & & & \multicolumn{3}{c|}{Warm} & \multicolumn{5}{c}{Cold} \\
          & & & & & & \multicolumn{3}{c|}{Item} & \multicolumn{2}{c}{User} \\
          & & & \mlonem & \onion & \amazonvid & \mlonem & \onion & \amazonvid &  \mlonem & \onion \\\midrule
          
\multirow{2}{*}{\baserec} & \multirow{1}{*}{\rand} & \apten & 0.0009 & 0.0003 & 0.0008 & 0.0101 & 0.0026 & 0.0065 & 0.0011 & 0.0003 \\
 & \multirow{1}{*}{\pop} & \apten & 0.0360 & 0.0056 & 0.0169 & 0.0011 & 0.0016 & 0.0099 & 0.0337 & 0.0056 \\
\midrule
\multirow{2}{*}{\cfbr} & \multirow{1}{*}{\mf} & \apten & 0.0924 & 0.0739 & \bfseries 0.0618$\dagger$ & 0.0048 & 0.0011 & 0.0077 & 0.0332 & 0.0048 \\
 & \multirow{1}{*}{\dmf} & \apten & 0.0312 & 0.0615 & 0.0392 & 0.0012 & 0.0058 & 0.0099 & 0.0272 & 0.0026 \\
\midrule
\multirow{5}{*}{\cbr} & \multirow{1}{*}{\dropoutnetTwo} & \apten & 0.0850 & 0.0305 & 0.0250 & 0.0629 & 0.0476 & 0.0675 & 0.0331 & 0.0058 \\
 & \multirow{1}{*}{\dropoutnetBest} & \apten & 0.0850 & 0.0408 & 0.0313 & 0.0629 & 0.0777 & 0.0675 & 0.0331 & \bfseries 0.0072 \\
 & \multirow{1}{*}{\clcrec} & \apten & \bfseries 0.0975 & 0.0726 & 0.0405 & 0.0498 & 0.0753 & 0.0974 & 0.0329 & 0.0055 \\
 & \multirow{1}{*}{\sbrecTwo} & \apten & 0.0948 & 0.0718 & 0.0523 & 0.0898 & 0.0682 & \bfseries 0.1054$\dagger$ & \bfseries 0.0343 & 0.0054 \\
 & \multirow{1}{*}{\sbrecBest} & \apten & 0.0947 & \bfseries 0.0780$\dagger$ & 0.0523 & \bfseries 0.1134$\dagger$ & \bfseries 0.0941$\dagger$ & \bfseries 0.1054$\dagger$ & 0.0330 & 0.0068 \\
 
        \bottomrule
    \end{tabular}}
    \vspace{0.6em}
    \caption{Evaluation results \wrt \apten. Bold indicates the best performing RS, $\dagger$ indicates significant improvement over allothers (paired $t$-tests with $p<0.05$ considering Bonferroni correction).}
    \label{tab:results-coverage}
\end{table*}
\end{center}

==> tables/tab_results_coverage.tex <==
\begin{center}
\begin{table*}[!htb]\scalebox{0.9}{
    \centering
    \begin{tabular}{lll|rrr|rrr|rr}
        %\toprule
          & & & \multicolumn{3}{c|}{Warm} & \multicolumn{5}{c}{Cold} \\
          & & & & & & \multicolumn{3}{c|}{Item} & \multicolumn{2}{c}{User} \\
          & & & \mlonem & \onion & \amazonvid & \mlonem & \onion & \amazonvid &  \mlonem & \onion \\\midrule
          
\multirow{2}{*}{\baserec} & \multirow{1}{*}{\rand} & \covten & \bfseries 1.0000 & \bfseries 0.9822 & \bfseries 1.0000 & \bfseries 1.0000 & \bfseries 1.0000 & \bfseries 1.0000 & \bfseries 0.8555 & \bfseries 0.3847 \\
 & \multirow{1}{*}{\pop} & \covten & 0.0288 & 0.0024 & 0.0041 & 0.0303 & 0.0073 & 0.0239 & 0.0032 & 0.0009 \\
\midrule
\multirow{2}{*}{\cfbr} & \multirow{1}{*}{\mf} & \covten & 0.5156 & 0.4712 & 0.7575 & 0.0303 & 0.0073 & 0.0239 & 0.0032 & 0.0009 \\
 & \multirow{1}{*}{\dmf} & \covten & 0.3741 & 0.3705 & 0.8875 & 0.0303 & 0.0073 & 0.0239 & 0.0032 & 0.0009 \\
\midrule
\multirow{5}{*}{\cbr} & \multirow{1}{*}{\dropoutnetTwo} & \covten & 0.4019 & 0.2996 & 0.1185 & 0.8697 & 0.8156 & 0.9737 & 0.0032 & 0.0028 \\
 & \multirow{1}{*}{\dropoutnetBest} & \covten & 0.4019 & 0.4059 & 0.4587 & 0.8697 & 0.8905 & 0.9737 & 0.0032 & 0.0055 \\
 & \multirow{1}{*}{\clcrec} & \covten & 0.4765 & 0.4417 & 0.8667 & 0.6667 & 0.9993 & \bfseries 1.0000 & 0.0055 & 0.0009 \\
 & \multirow{1}{*}{\sbrecTwo} & \covten & 0.5008 & 0.6663 & 0.7204 & 0.9606 & 0.9721 & 0.9928 & 0.0055 & 0.0186 \\
 & \multirow{1}{*}{\sbrecBest} & \covten & 0.4986 & 0.5405 & 0.7204 & 0.7636 & 0.9625 & 0.9928 & 0.0100 & 0.0087 \\
 
        \bottomrule
    \end{tabular}}
    \vspace{0.6em}
    \caption{Evaluation results \wrt \covten. Bold indicates the best performing RS. 
    }
    \label{tab:results-coverage}
\end{table*}
\end{center}

==> tables/tab_results_precision.tex <==
\begin{center}
\begin{table*}[!htb]\scalebox{0.9}{
    \centering
    \begin{tabular}{lll|rrr|rrr|rr}
          & & & \multicolumn{3}{c|}{Warm} & \multicolumn{5}{c}{Cold} \\
          & & & & & & \multicolumn{3}{c|}{Item} & \multicolumn{2}{c}{User} \\
          & & & \mlonem & \onion & \amazonvid & \mlonem & \onion & \amazonvid &  \mlonem & \onion \\\midrule
          
\multirow{2}{*}{\baserec} & \multirow{1}{*}{\rand} & \precten & 0.0048 & 0.0007 & 0.0003 & 0.0463 & 0.0061 & 0.0033 & 0.0455 & 0.0083 \\
 & \multirow{1}{*}{\pop} & \precten & 0.1016 & 0.0136 & 0.0059 & 0.0076 & 0.0056 & 0.0077 & 0.4380 & 0.0927 \\
\midrule
\multirow{2}{*}{\cfbr} & \multirow{1}{*}{\mf} & \precten & 0.2011 & 0.0818 & \bfseries 0.0158 & 0.0292 & 0.0054 & 0.0035 & 0.4424 & 0.0858 \\
 & \multirow{1}{*}{\dmf} & \precten & 0.0989 & 0.0793 & 0.0118 & 0.0090 & 0.0150 & 0.0077 & 0.4253 & 0.0581 \\
\midrule
\multirow{5}{*}{\cbr} & \multirow{1}{*}{\dropoutnetTwo} & \precten & 0.1884 & 0.0505 & 0.0083 & 0.1854 & 0.0791 & 0.0276 & 0.4395 & 0.0912 \\
 & \multirow{1}{*}{\dropoutnetBest} & \precten & 0.1884 & 0.0602 & 0.0095 & 0.1854 & 0.1109 & 0.0276 & 0.4395 & 0.1008 \\
 & \multirow{1}{*}{\clcrec} & \precten & \bfseries 0.2069$\dagger$ & 0.0764 & 0.0119 & 0.1644 & 0.0890 & 0.0314 & 0.4428 & 0.0927 \\
 & \multirow{1}{*}{\sbrecTwo} & \precten & 0.1983 & 0.0893 & 0.0151 & 0.2108 & 0.0900 & \bfseries 0.0355$\dagger$ & 0.4497 & 0.0852 \\
 & \multirow{1}{*}{\sbrecBest} & \precten & 0.1941 & \bfseries 0.1006$\dagger$ & 0.0151 & \bfseries 0.2350$\dagger$ & \bfseries 0.1301$\dagger$ & \bfseries 0.0355$\dagger$ & \bfseries 0.4534 & \bfseries 0.1025 \\

 
        \bottomrule
    \end{tabular}}
    \vspace{0.6em}
    \caption{Evaluation results \wrt \precten. Bold indicates the best performing RS, $\dagger$ indicates significant improvement over all others (paired $t$-tests with $p<0.05$ considering Bonferroni correction).
    }
    \label{tab:results-ndcg}
\end{table*}
\end{center}

==> tables/tab_results_recall.tex <==
\begin{center}
\begin{table*}[!htb]\scalebox{0.9}{
    \centering
    \begin{tabular}{lll|rrr|rrr|rr}
        %\toprule
          & & & \multicolumn{3}{c|}{Warm} & \multicolumn{5}{c}{Cold} \\
          & & & & & & \multicolumn{3}{c|}{Item} & \multicolumn{2}{c}{User} \\
          & & & \mlonem & \onion & \amazonvid & \mlonem & \onion & \amazonvid &  \mlonem & \onion \\\midrule

\multirow{2}{*}{\baserec} & \multirow{1}{*}{\rand} & \recten & 0.0031 & 0.0011 & 0.0026 & 0.0310 & 0.0087 & 0.0223 & 0.0034 & 0.0011 \\
 & \multirow{1}{*}{\pop} & \recten & 0.0798 & 0.0170 & 0.0515 & 0.0032 & 0.0064 & 0.0518 & 0.0508 & 0.0128 \\
\midrule
\multirow{2}{*}{\cfbr} & \multirow{1}{*}{\mf} & \recten & 0.1806 & 0.1438 & \bfseries 0.1394 & 0.0152 & 0.0056 & 0.0232 & 0.0520 & 0.0116 \\
 & \multirow{1}{*}{\dmf} & \recten & 0.0774 & 0.1224 & 0.1036 & 0.0042 & 0.0167 & 0.0518 & 0.0510 & 0.0079 \\
\midrule
\multirow{5}{*}{\cbr} & \multirow{1}{*}{\dropoutnetTwo} & \recten & 0.1666 & 0.0704 & 0.0743 & 0.1521 & 0.1144 & 0.1906 & 0.0517 & 0.0137 \\
 & \multirow{1}{*}{\dropoutnetBest} & \recten & 0.1666 & 0.0897 & 0.0834 & 0.1521 & 0.1618 & 0.1906 & 0.0517 & \bfseries 0.0155 \\
 & \multirow{1}{*}{\clcrec} & \recten & \bfseries 0.1851 & 0.1363 & 0.1051 & 0.1153 & 0.1169 & 0.2199 & 0.0527 & 0.0128 \\
 & \multirow{1}{*}{\sbrecTwo} & \recten & 0.1836 & 0.1449 & 0.1328 & 0.1736 & 0.1205 & \bfseries 0.2466$\dagger$ & \bfseries 0.0529 & 0.0121 \\
 & \multirow{1}{*}{\sbrecBest} & \recten & 0.1806 & \bfseries 0.1568$\dagger$ & 0.1328 & \bfseries 0.1869$\dagger$ & \bfseries 0.1904$\dagger$ & \bfseries 0.2466$\dagger$ & 0.0522 & 0.0146 \\

 
        \bottomrule
    \end{tabular}}
    \vspace{0.6em}
    \caption{Evaluation results \wrt \recten. Bold indicates the best performing RS% and the best performing \cbr model
    , $\dagger$ indicates significant improvement %of the best performing RS 
    over all %the 
    others (paired $t$-tests with $p<0.05$ considering Bonferroni correction).
    }
    \label{tab:results-recall}
\end{table*}
\end{center}
